Dynamic gNodeB Sleep Control for Energy-Conserving 5G Radio Access Network

5G radio access network (RAN) is consuming much more energy than legacy RAN due to the denser deployments of gNodeBs (gNBs) and higher single-gNB power consumption. In an effort to achieve an energy-conserving RAN, this paper develops a dynamic on-off switching paradigm, where the ON/OFF states of gNBs can be dynamically configured according to the evolvements of the associated users. We formulate the dynamic sleep control for a cluster of gNBs as a Markov decision process (MDP) and analyze various switching policies to reduce the energy expenditure. The optimal policy of the MDP that minimizes the energy expenditure can be derived from dynamic programming, but the computation is expensive. To circumvent this issue, this paper puts forth a greedy policy and an index policy for gNB sleep control. When there is no constraint on the number of gNBs that can be turned off, we prove the dual-threshold structure of the greedy policy and analyze its connections with the optimal policy. Inspired by the dual-threshold structure and Whittle index, we develop an index policy by decoupling the original MDP into multiple one-dimensional MDPs -- the indexability of the decoupled MDP is proven and an algorithm to compute the index is proposed. Extensive simulation results verify that the index policy exhibits close-to-optimal performance in terms of the energy expenditure of the gNB cluster. As far as the computational complexity is concerned, on the other hand, the index policy is much more efficient than the optimal policy, which is computationally prohibitive when the number of gNBs is large.

==> Notes.tex <==
This file is used to take notes.

%%%%%   \mathcal{}
%%%%%   {\mathcal P}_\text{static}
%%%%%   \mathbb{}
%%%%%   \overline{}
%%%%%   \triangleq
%%%%%   \bar{C}_\pi
%%%%%   ``...''
%%%%%   '
%%%%%   \eqref  \ref    \cite
%%%%%   \ref~
%%%%%   \eqnarray
%%%%%   nonumber
%%%%%   ^\prime
%%%%%   \overset{a}{=}
%%%%%   --
%%%%%   how to represent (M,0)?
%%%%%   \epsilon^*
%%%%%   $$...$$
%%%%%   \widetilde
%%%%%   
%%%%%   monotonously monotonically increasing







% \begin{eqnarray*}
%     \hspace{-0.7cm} && h(\widetilde{n},\Gamma^{L1},\Gamma^U)-h(\widetilde{n},\Gamma^{L2},\Gamma^U)=\\
%     \hspace{-0.7cm} && \begin{cases}
%         0-0=0,& \widetilde{n} \le \Gamma^{L1};\\
%         \Delta_2 (\widetilde{n}) + F(\Gamma^{L1},\Gamma^U)-0 \le 0,& \Gamma^{L1} < \widetilde{n} \le \Gamma^{L2};\\
%         \Delta_2 (\widetilde{n}) + F(\Gamma^{L1},\Gamma^U) - \\
%         \Delta_2 (\widetilde{n}) - F(\Gamma^{L2},\Gamma^U) \overset{(a)}{\le} 0 ,
%         & \Gamma^{L2} < \widetilde{n} \le \Gamma^U;\\
%         \Delta_1 (\widetilde{n})-\Delta_1 (\widetilde{n})=0,& \widetilde{n} > \Gamma^U,
%     \end{cases}
% \end{eqnarray*}
% where $(a)$ follows because
% \begin{eqnarray*}
%     && \Delta_2 (\widetilde{n}) + F(\Gamma^{L1},\Gamma^U) - \Delta_2 (\widetilde{n}) - F(\Gamma^{L2},\Gamma^U) \\
%     = && F(\Gamma^{L1},\Gamma^U) - F(\Gamma^{L2},\Gamma^U) \\
%     \overset{(a)}{=} && -\Delta_2 (\Gamma^{L1}) + \Delta_2 (\Gamma^{L2}) \overset{(b)}{\le} 0,
% \end{eqnarray*}
% where $(a)$ can be achieved from \eqref{eqF1_1}, $(b)$ follows because $\Delta_2$ is a monotonically non-increasing function and $\Gamma^{L1}<\Gamma^{L2}$. As a result, we get
% $h(\widetilde{n},\Gamma^{L1},\Gamma^U)-h(\widetilde{n},\Gamma^{L2},\Gamma^U) \le 0, \Gamma^{L1}<\Gamma^{L2}$, i.e., $h(\widetilde{n},\Gamma^L,\Gamma^U)$ is a monotonically non-increasing function with $\Gamma^L$.

% For $\Gamma^{U1}<\Gamma^{U2}$, we have
% \begin{eqnarray}\label{eqF1_2}
%     \hspace{-0.7cm} && h(\widetilde{n},\Gamma^L,\Gamma^{U1})-h(\widetilde{n},\Gamma^L,\Gamma^{U2})=\\
%     \hspace{-0.7cm} && \begin{cases}
%         0-0=0,& \widetilde{n} \le \Gamma^L;\\
%         \Delta_2 (\widetilde{n}) + F(\Gamma^L,\Gamma^{U1}) - \\
%         \Delta_2 (\widetilde{n}) - F(\Gamma^L,\Gamma^{U2}) \overset{(a)}{\le} 0 ,
%         & \Gamma^L < \widetilde{n} \le \Gamma^{U1};\\
%         \Delta_1 (\widetilde{n}) - \Delta_2 (\widetilde{n}) - F(\Gamma^L,\Gamma^{U2}) \overset{(b)}{\le} 0,& \Gamma^{U1} < \widetilde{n} \le \Gamma^{U2};\\
%         \Delta_1 (\widetilde{n})-\Delta_1 (\widetilde{n})=0,& \widetilde{n} > \Gamma^{U2},\\
%     \end{cases} \nonumber
% \end{eqnarray}
% where $(a)$ follows because
% \begin{eqnarray*}
%     && \Delta_2 (\widetilde{n}) + F(\Gamma^L,\Gamma^{U1}) - \Delta_2 (\widetilde{n}) - F(\Gamma^L,\Gamma^{U2}) \\
%     = && F(\Gamma^L,\Gamma^{U1}) - F(\Gamma^L,\Gamma^{U2}) \\
%     = && \Delta_1 (\Gamma^{U1})-\Delta_2 (\Gamma^{U1}) - \Delta_1 (\Gamma^{U2})+\Delta_2 (\Gamma^{U2}),
% \end{eqnarray*}
% as
% \begin{eqnarray*}
%     \Delta_1 (\Gamma^U)-\Delta_2 (\Gamma^U) = && \hspace{-0.5cm} f\left[ {(\Gamma^U+\overline{\lambda} T_s ) \cdot {\mathcal{P}}_e } \right] - \\
%     && \hspace{-0.5cm} f\left[ {{\mathcal{P}}_\text{static}+{\mathcal{P}}_\text{switch}+( \Gamma^U+\overline{\lambda} T_s ) \cdot {\mathcal{P}}_d } \right] \\
%     = && \hspace{-0.5cm} g^U(\Gamma^U)
% \end{eqnarray*}
% is a monotonically increasing function, thus we have $\Delta_1 (\Gamma^{U1})-\Delta_2 (\Gamma^{U1}) - \Delta_1 (\Gamma^{U2})+\Delta_2 (\Gamma^{U2})<0$ when $\Gamma^{U1}<\Gamma^{U2}$, i.e. $(a)$ in \eqref{eqF1_2} follows. $(b)$ in \eqref{eqF1_2} follows because
% \begin{eqnarray*}
%     \Delta_1 (\widetilde{n}) - \Delta_2 (\widetilde{n}) - F(\Gamma^L,\Gamma^{U2}) \\
%     = g^U(\widetilde{n}) - F(\Gamma^L,\Gamma^{U2}),
% \end{eqnarray*}
% as $g^U$ is a monotonically increasing function, and $g^U(\Gamma^{U2}) = F(\Gamma^L,\Gamma^{U2}) $ from \eqref{eqE7}, we can get $g^U(\widetilde{n}) - F(\Gamma^L,\Gamma^{U2}) \le 0$ when $\widetilde{n} \le \Gamma^{U2}$, i.e., $(b)$ in \eqref{eqF1_2} follows.

% As shown in Fig.~\ref{}, when $\Gamma^L$ or $\Gamma^U$ becomes larger, the values for each $h(\widetilde{n})$ will become larger or keep constant. As a result, $H$ in \eqref{eqF2} is monotonically non-decreasing with $\Gamma^L$ and $\Gamma^U$.

















% Note that $\Gamma^L$ and $\Gamma^U$ are both functions of $\epsilon$, and we have the following Lemma.

% \begin{lem}[Same monotonicity of $\Gamma^L(\epsilon)$ and $\Gamma^U(\epsilon)$] \label{lem_same_monotonicity}
% $\Gamma^L(\epsilon)$ and $\Gamma^U(\epsilon)$ have the same monotonicity with $\epsilon$.
% \end{lem}

% \begin{NewProof}
% We first rewrite \eqref{eqE6} and \eqref{eqE7} below:
% \begin{eqnarray}\label{eqF5}
%     \begin{cases}
%         g^L\left[\Gamma^L(\epsilon) \right] = - \epsilon + H\left[\Gamma^L(\epsilon),\Gamma^U(\epsilon) \right], \\
%         g^U\left[\Gamma^U(\epsilon) \right] = - \epsilon + H\left[\Gamma^L(\epsilon),\Gamma^U(\epsilon) \right].
%     \end{cases}
% \end{eqnarray}
% where $g^L\left(\cdot\right)$ and $g^U\left(\cdot\right)$ are both monotonically increasing functions. It can also be noted from \eqref{eqF4} that for a given $\epsilon$, we have
% \begin{equation*}
%     g^L\left[\Gamma^L(\epsilon) \right] = g^U\left[\Gamma^U(\epsilon)\right],
% \end{equation*}
% as they are both equal to a same expression. As a result, for $\epsilon_1 \ne \epsilon2$, if $\Gamma^L(\epsilon_1)>\Gamma^L(\epsilon_2)$, then $g^L\left( \Gamma^L(\epsilon_1) \right) > g^L\left( \Gamma^L(\epsilon_2) \right)$ and also $g^U\left( \Gamma^U(\epsilon_1) \right) > g^U\left( \Gamma^U(\epsilon_2) \right)$, thus $\Gamma^U(\epsilon_1)>\Gamma^U(\epsilon_2)$; on the other hand, if $\Gamma^L(\epsilon_1)<\Gamma^L(\epsilon_2)$, we can get $\Gamma^U(\epsilon_1)<\Gamma^U(\epsilon_2)$. That is to say, $\Gamma^L(\epsilon)$ and $\Gamma^U(\epsilon)$ have the same monotonicity with $\epsilon$.
% \end{NewProof}

% Based on Lemma~\ref{lem_H_monotone_nondecreasing}~and~\ref{lem_same_monotonicity}, we can show the monotonically decreasing property of $\Gamma^L(\epsilon)$ and $\Gamma^U(\epsilon)$ next.
% \begin{lem}[Monotonically decreasing of $\Gamma^L(\epsilon)$ and $\Gamma^U(\epsilon)$] \label{lem_Gamma_monotone_decreasing}
% $\Gamma^L(\epsilon)$ and $\Gamma^U(\epsilon)$ are both monotonically decreasing with $\epsilon$. And then decoupled problem defined in Definition~\ref{defi_decoupled_problem} is indexable.
% \end{lem}

% \begin{NewProof}
% We first show $\Gamma^L(\epsilon)$ and $\Gamma^U(\epsilon)$ are both monotonically decreasing. According to Lemma~\ref{lem_same_monotonicity}, we only need to prove that $\Gamma^U(\epsilon)$ is monotonically decreasing with $\epsilon$.
% \begin{enumerate}
%     \item When $\epsilon \ge -g^U(0)$, we have
%     \begin{eqnarray*}
%         g^U\left[\Gamma^U(\epsilon) \right] &=& - \epsilon + H\left[\Gamma^L(\epsilon),\Gamma^U(\epsilon) \right] \\
%         &\le& g^U(0) + 0 = g^U(0).
%     \end{eqnarray*}
    
%     As $g^U(\cdot)$ is a monotonically increasing function, we can get $\Gamma^U(\epsilon) \le 0$, thus $\widetilde{n} \ge \Gamma^U(\epsilon), \forall \widetilde{n} \ge 0 $, so $H=E$ is a constant, where $E$ is defined in \eqref{eqF3}. At this time, $g^U\left( \Gamma^U(\epsilon) \right) = -\epsilon + E$ is monotonically decreasing with $\epsilon$, so $\Gamma^U(\epsilon)$ is also monotonically decreasing with $\epsilon$.
    
%     \item When $\epsilon < -g^U(0)$, for $\forall \epsilon_1 < \epsilon_2 < -\Gamma^U(0)$, we have
%     \begin{eqnarray}\label{eqF6}
%         g^U\left[ \Gamma^U(\epsilon_1) \right] &=& -\epsilon_1 + H\left[ \Gamma^L(\epsilon_1),\Gamma^U(\epsilon_1) \right] \nonumber \\
%         &>& -\epsilon_2 + H\left[ \Gamma^L(\epsilon_1),\Gamma^U(\epsilon_1) \right] \nonumber \\
%         &\triangleq& g^U\left[ \Gamma^U(\epsilon_{(1)}) \right],
%     \end{eqnarray}
%     where $\Gamma^U(\epsilon_{(1)})$ is a new defined variable. According to the monotonically increasing property of $g^U(\cdot)$, we have $\Gamma^U(\epsilon_{(1)}) < \Gamma^U(\epsilon_1)$, and $\Gamma^L(\epsilon_{(1)}) < \Gamma^L(\epsilon_1)$ can be achieved because of Lemma~\ref{lem_same_monotonicity}. Then we have
%     \begin{eqnarray*}
%         g^U\left[ \Gamma^U(\epsilon_{(1)}) \right] &=& -\epsilon_2 + H\left[ \Gamma^L(\epsilon_1),\Gamma^U(\epsilon_{(1)}) \right] \\
%         &\overset{(a)}{>}& -\epsilon_2 + H\left[ \Gamma^L(\epsilon_{(1)}),\Gamma^U(\epsilon_{(1)}) \right] \\
%         &\triangleq& g^U\left[ \Gamma^U(\epsilon_{(2)}) \right],
%     \end{eqnarray*}
%     where $(a)$ follows because $H$ is a monotonically non-decreasing function with $\Gamma^L$ and $\Gamma^U$, as shown in Lemma~\ref{lem_H_monotone_nondecreasing}. In this way, we can construct a sequence $\left\{ {\Gamma^U(\epsilon_{(i)}), i=1,2,\cdots} \right\}$, in which $\left\{ {\Gamma^U(\epsilon_{(1)})} \right\}$ is defined in \eqref{eqF6}, and the others follow:
%     \begin{eqnarray}\label{eqF7}
%         g^U\left[ \Gamma^U(\epsilon_{(i)}) \right] \hspace{-0.3cm} &=& \hspace{-0.3cm} -\epsilon_2 + H\left[ \Gamma^L(\epsilon_{(i-1)}),\Gamma^U(\epsilon_{(i-1)}) \right] \nonumber \\
%         &\overset{(a)}{>}& -\epsilon_2 + H\left[ \Gamma^L(\epsilon_{(i)} ),\Gamma^U(\epsilon_{(i)}) \right] \nonumber \\
%         &=& g^U\left[ \Gamma^U(\epsilon_{(i+1)}) \right], \nonumber\\
%         i &=& 2,3,\cdots
%     \end{eqnarray}
%     where $(a)$ can be achieved using mathematical induction. As a result, $\left\{ {\Gamma^U(\epsilon_{(i)}), i=1,2,\cdots} \right\}$ is a monotonically decreasing sequence, and for $\forall i \ge 2$, it satisfies
%     \begin{eqnarray*}
%         g^U\left[ \Gamma^U(\epsilon_{(i)}) \right] \hspace{-0.3cm} &=& \hspace{-0.3cm} -\epsilon_2 + H\left[ \Gamma^L(\epsilon_{(i-1)}),\Gamma^U(\epsilon_{(i-1)}) \right] \\
%         &>& g^U\left(0\right) + E,
%     \end{eqnarray*}
%     which means that the sequence $\left\{ {\Gamma^U(\epsilon_{(i)})} \right\}$ has a lower bound. Combining with the fact that it is a monotonically decreasing sequence, we can conclude that its limit exists and can be represented by $\Gamma^U(\epsilon_{(\infty)})$. According to \eqref{eqF7}, we can get
%     \begin{equation*}
%         g^U\left[ \Gamma^U(\epsilon_{(\infty)}) \right] = -\epsilon_2 + H\left[ \Gamma^L\left(\epsilon_{(\infty)} \right),\Gamma^U\left(\epsilon_{(\infty)} \right) \right].
%     \end{equation*}
    
%     Note that $g^U\left[ \Gamma^U\left(\epsilon_2 \right) \right] = -\epsilon_2 + H\left[ \Gamma^L\left(\epsilon_2 \right),\Gamma^U\left(\epsilon_2 \right) \right]$ according to \eqref{eqF5}, so we get $\epsilon_{(\infty)} = \epsilon_2$. Then we have
%     \begin{equation}\label{F8}
%         \Gamma^U\left(\epsilon_2\right) = \Gamma^U(\epsilon_{(\infty)})
%         \overset{(a)}{<} \Gamma^U\left(\epsilon_{(1)}\right)
%         \overset{(b)}{<} \Gamma^U\left(\epsilon_1\right) ,
%     \end{equation}
%     where $(a)$ follows because $\left\{ {\Gamma^U\left(\epsilon_{(i)}\right)} \right\}$ is a monotonically decreasing sequence; $(b)$ follows from \eqref{eqF6}. As a result, we get $\Gamma^U\left(\epsilon_2\right) < \Gamma^U\left(\epsilon_1\right)$ for $\forall \epsilon_1 < \epsilon_2 < -\Gamma^U\left(0\right)$, i.e., $\Gamma^U\left(\epsilon \right)$ is monotonically decreasing with $\epsilon$.
% \end{enumerate}

% In this way, we show the monotonically decreasing property of $\Gamma^U\left(\epsilon \right)$, thus $\Gamma^L\left(\epsilon \right)$ is also monotonically decreasing with $\epsilon$ from Lemma~\ref{lem_same_monotonicity}. As a result, the passive set $D\left( \epsilon \right)$ defined in \eqref{eqE8} is monotonically non-increasing with $\epsilon$, so the decoupled problem is indexable.
% \end{NewProof}
